Distributed Submodular Maximization with Parallel Execution

The submodular maximization problem is widely applicable in many engineering problems where objectives exhibit diminishing returns. While this problem is known to be NP-hard for certain subclasses of objective functions, there is a greedy algorithm which guarantees approximation at least 1/2 of the optimal solution. This greedy algorithm can be implemented with a set of agents, each making a decision sequentially based on the choices of all prior agents. In this paper, we consider a generalization of the greedy algorithm in which agents can make decisions in parallel, rather than strictly in sequence. In particular, we are interested in partitioning the agents, where a set of agents in the partition all make a decision simultaneously based on the choices of prior agents, so that the algorithm terminates in limited iterations. We provide bounds on the performance of this parallelized version of the greedy algorithm and show that dividing the agents evenly among the sets in the partition yields an optimal structure. We additionally show that this optimal structure is still near-optimal when the objective function exhibits a certain monotone property. Lastly, we show that the same performance guarantees can be achieved in the parallelized greedy algorithm even when agents can only observe the decisions of a subset of prior agents.

==> limited-communication.tex <==
\section{Limited Communication}
\begin{cor}
Given any graph $G = (V, E)$ so that $\gamma(G) \ge 1/(k+1)$ for some integer $k > 1$, then
\begin{equation}
\begin{aligned}
    |E| &\ge \frac{1}{2}(n \mod{k}) \left\lceil \frac{n}{k} \right\rceil \left(\left\lceil \frac{n}{k} \right\rceil - 1\right)\\
    &\phantom{==}+ \frac{1}{2}(-n \mod{k}) \left\lfloor \frac{n}{k} \right\rfloor \left(\left\lfloor \frac{n}{k} \right\rfloor - 1\right)
\end{aligned}
\end{equation}
where $n = |V|$.
Furthermore, the complement Tur\`{a}n graph $\overline{T(n; k)}$ achieves this lower bound.
\end{cor}

\begin{definition}
A distributed submodular maximization problem satisfies \textit{$p$-wise redundancy constraint} if there is some nonnegative function $\Phi$ so that for all $A \subseteq V$ where $|A| = p$,
\begin{equation}
    \sum_{i \in A} f(x_i) \geq f\left(\{x_i\}_{i \in A}\right) \geq \Phi\left( \{f(x_i)\}_{i \in A}, f\left(\{x_i\}_{i \in A}\right) \right).
\end{equation}
We say the problem is \textit{$p$-additive} if the inequalities above are equalities.
\end{definition}

Note that $\beta$-strict montonicity is a $p$-wise redundancy constraint for all positive integer $p$.

\begin{definition}
Let $\gamma_p(G)$ be the efficiency guarantee of $G$ subject to $p$-additivity. Formally,
\begin{equation}
    \gamma_p(G) = \inf_{(f, X) \text{ are $p$-additive}} \gamma(f, X, G)
\end{equation}
\end{definition}

\begin{theorem}
\label{thm:not-useful}
    Given any graph $G = (V, E)$ so that $\gamma_p(G) \ge 1/(k+1)$ for some fixed integers $p \ge 1$ and $k > 1$, then
    \begin{equation}
        |E| \ge \left(\frac{1}{k} + o(1)\right)\binom{n}{2}
    \end{equation}
    as a function of $n$, where $n = |V|$.
    Furthermore, the complement Tur\`{a}n graph $\overline{T(n; k)}$ achieves this lower bound asymptotically.
\end{theorem}

\subsection{Proof of Theorem \ref{thm:not-useful}}
To prove Theorem \ref{thm:not-useful}, we will show an upper bound on $\gamma_p$ with an explicit construction.
First, we will need a few definitions which will be key to the construction.
\begin{definition}
\label{def:p-indep}
A set of nodes $J$ is called \textit{$p$-pseudo-independent} if for every $j \in J$, $|\mathcal{N}_j \cap J| < p$. 
The \textit{$p$-pseudo-independent} number $\alpha_p(G)$ is the size of the maximum $p$-pseudo-independent set.
\end{definition}

\begin{definition}
\label{def:p-sib}
A node $w$ is a \textit{$p$-sibling} of a maximum $p$-pseudo-independent set $J$ if $w \in V \setminus J$ and there exist distinct $j_1, \dots, j_p \in J$ s.t. $j_i \in \mathcal{N}_w$.
And a graph $G$ has the \textit{$p$-sibling property} if some maximum $p$-pseudo-independent set in $G$ has a $p$-sibling.
\end{definition}

\begin{lemma}
\label{thm:no-sibling}
If a graph $G$ does not have the $p$-sibling property, then it has no disjoint maximum $p$-pseudo-independent sets. 
\end{lemma}

\begin{proof}
Suppose the contrary, there are maximum pseudo-independent sets $J, J'$ so that $J' \cap J = \emptyset$.
Let $j= \max(J \cup J')$ be the last node in $J$ and $J'$ and WLOG $j \in J'$.
For any $i \in J$, $|\mathcal{N}_i \cap (J \cup \{j\})| = |\mathcal{N}_i \cap J| < p$ since by definition $j \not\in \mathcal{N}_i$.
And because $j$ cannot be a $p$-sibling of $J$, $|\mathcal{N}_j \cap (J \cup \{j\})| \le |\mathcal{N}_j \cap J| < p$.
This implies that $J \cup \{j\}$ is $p$-pseudo-independent, contradiction.
\end{proof}

\begin{lemma}
\label{thm:upper-bound}
Given a graph $G$ with the $p$-sibling property, then 
\begin{equation}
    \gamma_p(G) \le \frac{p}{\alpha_p(G) + 1}
\end{equation}
and if $G$ does not have the $p$-sibling property, then
\begin{equation}
    \gamma_p(G) \le \frac{p}{\alpha_p(G)}
\end{equation}
\end{lemma}
\begin{proof}
We first consider the case with the sibling property.
Let $J$ be the maximum pseudo-independent set of $G$ with a sibling.
Let $a = \alpha_p(G)$ and denote $J_i$ be the $i$th node in $J$ and $J_{a+1}$ be a sibling of $J$.
Consider $S = \{u_1, \dots, u_a, v_1, \dots, v_a, w\}$ and action sets defined by:
\begin{equation}
X_{i} = 
\begin{cases}
    \{u_i, v_i\} & \text{if } i \in \{J_1, \dots, J_a\} \\
    \{u_i, t\} & \text{if } i = J_{a+1} \\
    \emptyset & \text{otherwise}
\end{cases}
\end{equation}

We now define the function $f : 2^S \to \mathbb{R}$ that for any $A \subseteq S$,
\begin{equation}
f(A) = \min\left(1, \sum_{u_i \in A} \frac{1}{p} \right) + \sum_{v_i \in A} \frac{1}{p}
\end{equation}

Note that through this construction, $f$ is monotonic, submodular, and $p$-additive.
$f$ also has the following properties for any $i \in \{J_1, \dots, J_a\}$:
\begin{enumerate}
    \item $f(u_i) = f(v_i) = 1/p$.
    \item $f(u_i \mid \cup_{j \in A} \{u_j\}) = f(u_i)$ for any $A \subseteq \mathcal{N}_i$ due to Definition \ref{def:p-indep}.
    \item $f(v_i | B) = f(v_i)$ for any $B \subseteq S \{i\}$
\end{enumerate}

Given these properties, it follows that in the greedy solution, the actions of $J_1, \dots, J_{a+1}$ are $u_1, u_2, \dots, u_a, t$, respectively.
And in the optimal solution, the actions of $J_1, \dots, J_{a+1}$ are $v_1, v_2, \dots, v_a, u_{a+1}$, respectively.
This results in $f(\xsol) \le 1$ and $f(\xopt) = a + 1$, hence $\gamma_p(G) \le p / (a+1)$.

The case without the sibling property follows the same construction, except that we do not have $J_{a+1}$.
This results in $f(\xsol) \le 1$ and $f(\xopt) = a$, leading to $\gamma_p(G) \le p / a$.
\end{proof}

The following result is also essential in the proof. 
\begin{theorem}[Erd\H{o}s-Stone \cite{erdos1946structure}]
Given a graph $H$, let $ex(n; H)$ be the maximum number of edges in an $n$-node graph not containing $H$.
Then 
\begin{equation}
    ex(n; H) = \left(1 - \frac{1}{\chi(H)-1} + o(1)\right) \binom{n}{2}
\end{equation}
as a function in $n$.
\end{theorem}

If we instead consider the complement, we can equivalently state the following.

\begin{cor}
\label{thm:erdos-stone}
Given a graph $H$, let $ex'(n; H)$ be the minimum number of edges in an $n$-node graph not containing $H$ or any of its spanning subgraph.
Then 
\begin{equation}
    ex'(n; H) = \left(\frac{1}{\theta(H)-1} + o(1)\right) \binom{n}{2}
\end{equation}
as a function in $n$.
\end{cor}

\begin{lemma}
\label{thm:min-edges}
Given a graph $G = (V, E)$, we have
\begin{equation}
    |E| \ge \left(\frac{1}{\lceil (\alpha_p(G) + 1) / m\rceil - 1} + o(1)\right)\binom{n}{2}
\end{equation}
\end{lemma}
\begin{proof}
Let $H$ be a graph with $\alpha_p(G) + 1$ nodes and edges $\{(i, j) \mid i \neq j, \lceil i/p \rceil = \lceil j / p\rceil\}$.
It is clear from the definition that $w(H) = \lceil (\alpha_p(G) + 1) / p \rceil$.
By Definition \ref{def:p-indep}, $G$ cannot contain $H$ or any of its spanning subgraphs.
Then this lemma immediately follows from Corollary \ref{thm:erdos-stone}.
\end{proof}

Now we complete the proof of Theorem \ref{thm:not-useful}. 
If $\alpha_p(G) > p(k+1)$, then by Lemma \ref{thm:upper-bound}, $\gamma_p(G) < 1/(k+1)$.
If $\alpha_p(G) = p(k+1)$ and $G$ has the $p$-sibling property, then by Lemma \ref{thm:upper-bound}, $\gamma_p(G) < 1/(k+1)$.
Hence we are interested in the following two cases:
\begin{enumerate}
    \item $\alpha_p(G) < p (k+1)$, with or without $m$-sibling property.
    \item $\alpha_p(G) = p (k+1)$ and no $m$-sibling property.
\end{enumerate}
In the first case, Lemma \ref{thm:min-edges} implies that $G$ has at least $(1/k + o(1))\binom{n}{2}$ edges.
And in the second case, let $J$ be a maximum $p$-pseudo-independent set of $G$.
Consider the graph $G'$ induced by removing all nodes in $J$ from $G$.
By Lemma \ref{thm:no-sibling}, $\alpha_p(G') < \alpha_p(G)$, and thus Lemma \ref{thm:min-edges} implies that the number of edges in $G'$ is at least 
\begin{subequations}
\begin{align}
    & \left(\frac{1}{k} + o(1)\right)\binom{n-p(k+1)}{2} \\
    ={}& \left(\frac{1}{k} + o(1)\right)\frac{n^2 - n + g(n)}{2} \label{equ:messy-expan} \\
    ={}& \left(\frac{1}{k} + o(1)\right)\binom{n}{2}
\end{align}
\end{subequations}
where $g(n)$ in \eqref{equ:messy-expan} is $-2p(k+1)n + p(k+1)(p(k+1)+1)$.

This theorem follows from combining the two above cases.


==> proof-parallel-beta.tex <==
\subsection{Extension of Theorem \ref{thm:best-parallel-strict-monotone} to Information Graphs}
\label{sec:proof-parallel-beta}


We will prove a version of Theorem \ref{thm:best-parallel-strict-monotone} generalized to information graphs, and the original theorem follows from the same logic.


\begin{theorem}
\label{thm:best-parallel-strict-monotone-graph}
    Given a parallelized submodular and $\beta$-strictly monotone maximization problem with $n$ agents and $q$ iterations, then:
    \begin{equation}
    \label{equ:strict-monotone-parallel-bounds-graph}
        \frac{(r-1)\beta+1}{r} \ge \eta'(n, q) \ge \frac{(r-1)\beta+1}{r - \beta + 1}
    \end{equation}
    Furthermore, the graph $G$ as defined in \eqref{equ:complement-turan} achieves the lower bound $\gamma'(G) \ge \frac{(r-1)\beta+1}{r - \beta + 1}$.
\end{theorem}

To prove Theorem \ref{thm:best-parallel-strict-monotone-graph}, we present a lower and an upper bound on the competitive ratio subject to $\beta$-strict monotoncity in a similar fashion as Lemma \ref{thm:david}.
The following lemma is proven in the Appendix.
\begin{lemma}
\label{thm:strict-monotone-lower}
Given any information graph $G$,
\begin{equation}
    \frac{(\alpha(G)-1)\beta + 1}{\alpha(G)} \ge \gamma'(G) \ge \frac{(\theta(G)-1)\beta + 1}{\theta(G) - \beta + 1}
\end{equation}

\end{lemma}

Now we come back to the proof of Theorem \ref{thm:best-parallel-strict-monotone-graph}.
The upper bound in \eqref{equ:strict-monotone-parallel-bounds-graph} follows from combining Lemma \ref{thm:parallel-indep-number} and the upper bound in Lemma \ref{thm:strict-monotone-lower}.
Consider the graph $G$ described by \eqref{equ:complement-turan}; as we already argued previously in Section \ref{sec:proof-parallel}, $r = \alpha(G) = \theta(G)$ and $G \in \mathcal{G}_{n, q}$.
Hence, from the lower bound in Lemma \ref{thm:strict-monotone-lower}, we conclude that this $G$ achieves the lower bound in \eqref{equ:strict-monotone-parallel-bounds-graph}, so we are done. \hfill$\blacksquare$

